The SOPHIE search for northern extrasolar planets. XVI. HD 158259: A compact planetary system in a near-3:2 mean motion resonance chain

Since 2011, the SOPHIE spectrograph has been used to search for Neptunes and super-Earths in the Northern Hemisphere. As part of this observational program, 290 radial velocity measurements of the 6.4 V magnitude star HD 158259 were obtained. Additionally, TESS photometric measurements of this target are available. We present an analysis of the SOPHIE data and compare our results with the output of the TESS pipeline. The radial velocity data, ancillary spectroscopic indices, and ground-based photometric measurements were analyzed with classical and $\ell_1$ periodograms. The stellar activity was modeled as a correlated Gaussian noise and its impact on the planet detection was measured with a new technique. The SOPHIE data support the detection of five planets, each with $m \sin i \approx 6 M_\oplus$, orbiting HD 158259 in 3.4, 5.2, 7.9, 12, and 17.4 days. Though a planetary origin is strongly favored, the 17.4 d signal is classified as a planet candidate due to a slightly lower statistical significance and to its proximity to the expected stellar rotation period. The data also present low frequency variations, most likely originating from a magnetic cycle and instrument systematics. Furthermore, the TESS pipeline reports a significant signal at 2.17 days corresponding to a planet of radius $\approx 1.2 R_\oplus$. A compatible signal is seen in the radial velocities, which confirms the detection of an additional planet and yields a $\approx 2 M_\oplus$ mass estimate. We find a system of five planets and a strong candidate near a 3:2 mean motion resonance chain orbiting HD 158259. The planets are found to be outside of the two and three body resonances.

==> parameters_evolution.tex <==

Parameter & ML fit & posterior mean & posterior median & 68.27\% confidence interval & 95.45\% confidence interval & 99.73\% confidence interval\\ \hline \hline  lin.offset& 13537.403138666& 13537.217105536& 13537.215143618& [13536.61 , 13537.76]& [13536.14 , 13538.51]& [13535.33 , 13539.07]\\ lin.smoothed rhk& -2.918945& -3.162538& -3.147721& [-3.638 , -2.618]& [-4.282 , -2.185]& [-4.877 , -1.494]\\ \hline  \multicolumn{7}{c}{Planet1}\\ \hline$P$ (d)& 3.4312293& 3.4312265& 3.4312231& [3.4304 , 3.4320]& [3.4296 , 3.4328]& [3.4287 , 3.4338]\\ $K$ (m/s) & 2.52315& 2.57975& 2.57657& [2.26 , 2.87]& [2.00 , 3.16]& [1.72 , 3.46]\\ $\lambda_0$ (rad) & 4.30954& 4.30793& 4.30488& [4.18 , 4.41]& [4.06 , 4.53]& [3.96 , 4.69]\\ $\sqrt{e} \cos \omega$ & 0.04470& 0.02026& 0.01818& [-0.08 , 0.09]& [-0.15 , 0.20]& [-0.24 , 0.27]\\ $\sqrt{e} \sin \omega$ & -0.09877& 0.00910& 0.00882& [-0.08 , 0.11]& [-0.17 , 0.19]& [-0.25 , 0.29]\\ \hline  \multicolumn{7}{c}{Planet2}\\ \hline$P$ (d)& 5.1382437& 5.1387871& 5.1389006& [5.1347 , 5.1430]& [5.130 , 5.146]& [5.126 , 5.149]\\ $K$ (m/s) & 1.50865& 1.47259& 1.47407& [1.13 , 1.75]& [0.82 , 2.11]& [0.50 , 2.62]\\ $\lambda_0$ (rad) & 0.08839& 2.80023& 0.42740& [0.00 , 6.04]& [0.02 , 6.28]& [0.00 , 6.28]\\ $\sqrt{e} \cos \omega$ & -0.03077& 0.00255& -0.00122& [-0.10 , 0.09]& [-0.18 , 0.19]& [-0.24 , 0.27]\\ $\sqrt{e} \sin \omega$ & -0.07580& -0.01054& -0.00943& [-0.11 , 0.06]& [-0.19 , 0.18]& [-0.29 , 0.26]\\ \hline  \multicolumn{7}{c}{Planet3}\\ \hline$P$ (d)& 7.950180& 7.942521& 7.942741& [7.933 , 7.949]& [7.926 , 7.958]& [7.917 , 7.968]\\ $K$ (m/s) & 1.86785& 1.73760& 1.72523& [1.26 , 2.08]& [0.99 , 2.59]& [0.56 , 2.83]\\ $\lambda_0$ (rad) & 3.49343& 3.42883& 3.43280& [3.15 , 3.68]& [2.87 , 3.95]& [2.50 , 4.17]\\ $\sqrt{e} \cos \omega$ & 0.13032& 0.00489& 0.00323& [-0.10 , 0.08]& [-0.18 , 0.19]& [-0.27 , 0.27]\\ $\sqrt{e} \sin \omega$ & 0.07692& 0.00403& 0.00259& [-0.08 , 0.09]& [-0.18 , 0.18]& [-0.25 , 0.28]\\ \hline  \multicolumn{7}{c}{Planet4}\\ \hline$P$ (d)& 14.4451516& 14.4315920& 14.4311004& [14.407 , 14.452]& [14.385 , 14.477]& [14.35 , 14.50]\\ $K$ (m/s) & 2.26482& 1.93688& 1.94638& [1.46 , 2.46]& [0.92 , 2.91]& [0.41 , 3.41]\\ $\lambda_0$ (rad) & 5.53338& 5.55100& 5.57980& [5.32 , 5.83]& [5.04 , 6.11]& [0.06 , 6.26]\\ $\sqrt{e} \cos \omega$ & -0.14086& -0.00665& -0.00513& [-0.11 , 0.08]& [-0.20 , 0.18]& [-0.28 , 0.25]\\ $\sqrt{e} \sin \omega$ & 0.06935& -0.01026& -0.00865& [-0.11 , 0.07]& [-0.19 , 0.16]& [-0.27 , 0.23]\\ \hline  \multicolumn{7}{c}{Planet5}\\ \hline$P$ (d)& 17.5632052& 17.5703931& 17.5727709& [17.538 , 17.611]& [17.48 , 17.65]& [17.41 , 17.67]\\ $K$ (m/s) & 2.51099& 2.35589& 2.35107& [1.85 , 2.93]& [1.24 , 3.41]& [0.65 , 4.00]\\ $\lambda_0$ (rad) & 3.98159& 3.81756& 3.82610& [3.55 , 4.02]& [3.26 , 4.28]& [2.88 , 4.52]\\ $\sqrt{e} \cos \omega$ & -0.04327& -0.00716& -0.00860& [-0.10 , 0.07]& [-0.20 , 0.16]& [-0.26 , 0.25]\\ $\sqrt{e} \sin \omega$ & -0.01903& 0.01050& 0.00927& [-0.09 , 0.09]& [-0.18 , 0.18]& [-0.27 , 0.28]\\ \hline  \multicolumn{7}{c}{Planet6}\\ \hline$P$ (d)& 363.7284909& 365.0376702& 365.0527480& [364.30 , 365.93]& [363.21 , 366.62]& [362.71 , 367.75]\\ $K$ (m/s) & 1.34259& 1.57469& 1.55089& [0.61 , 2.44]& [0.00 , 3.07]& [0.00 , 3.89]\\ $\lambda_0$ (rad) & 6.26401& 3.05688& 3.05895& [0.00 , 3.69]& [0.01 , 6.12]& [0.00 , 6.27]\\ $\sqrt{e} \cos \omega$ & -0.08425& 0.00414& 0.00392& [-0.09 , 0.09]& [-0.20 , 0.19]& [-0.28 , 0.30]\\ $\sqrt{e} \sin \omega$ & 0.02940& -0.00557& -0.00476& [-0.09 , 0.09]& [-0.20 , 0.18]& [-0.28 , 0.28]\\ \hline  \multicolumn{7}{c}{Planet7}\\ \hline$P$ (d)& 2.17852065& 2.17814421& 2.17813108& [2.17768 , 2.17858]& [2.1773 , 2.1790]& [2.1769 , 2.1794]\\ $K$ (m/s) & 1.15029& 1.23919& 1.24609& [0.95 , 1.51]& [0.65 , 1.78]& [0.36 , 2.02]\\ $\lambda_0$ (rad) & 0.71468& 0.68830& 0.56540& [0.25 , 0.79]& [0.00 , 1.10]& [0.02 , 6.28]\\ $\sqrt{e} \cos \omega$ & -0.04064& 0.00039& 0.00040& [-0.09 , 0.09]& [-0.18 , 0.19]& [-0.29 , 0.27]\\ $\sqrt{e} \sin \omega$ & 0.03051& -0.00592& -0.00227& [-0.10 , 0.07]& [-0.17 , 0.18]& [-0.25 , 0.28]\\ \hline  \multicolumn{7}{c}{Planet8}\\ \hline$\sigma_W$ (d)& 0.47519& 0.86168& 0.86587& [0.46 , 1.18]& [0.17 , 1.51]& [0.02 , 1.75]\\ $\sigma_R$ (d)& 7.20048& 2.91630& 2.90469& [2.59 , 3.25]& [2.24 , 3.61]& [1.94 , 4.04]\\ $\tau$ (d)& 3.90951& 4.12794& 3.71458& [2.19 , 4.65]& [1.85 , 7.64]& [1.47 , 13.8]\\ 


$m\sin i$ ($M_\oplus$)& 6.26& 6.39& 6.39& [5.55 , 7.18]& [4.82 , 8.14]& [4.14 , 9.16]\\ 
$m\sin i$ ($M_\oplus$)& 4.28& 4.18& 4.17& [3.22 , 5.09]& [2.20 , 6.03]& [1.44 , 7.90]\\ 
$m\sin i$ ($M_\oplus$)& 6.13& 5.70& 5.65& [4.30 , 7.02]& [3.16 , 8.75]& [2.192 , 10.06]\\ 
$m\sin i$ ($M_\oplus$)& 9.07& 7.75& 7.77& [5.66 , 9.83]& [3.611 , 11.78]& [0.90 , 13.3]\\ 
$m\sin i$ ($M_\oplus$)& 10.74& 10.07& 10.04& [7.731 , 12.56]& [5.292 , 14.96]& [2.50 , 17.5]\\ 
$m\sin i$ ($M_\oplus$)& 15.7& 18.5& 18.2& [6.85 , 28.2]& [0.06 , 36.3]& [0.03 , 46.4]\\ 
$m\sin i$ ($M_\oplus$)& 2.45& 2.64& 2.63& [2.09 , 3.34]& [1.33 , 3.84]& [0.80 , 4.52]\\ 






Parameter & ML fit & posterior mean & posterior median & 68.27\% confidence interval & 95.45\% confidence interval & 99.73\% confidence interval\\ \hline \hline  lin.offset& 13538.414997016& 13538.296390057& 13538.335517413& [13537.71 , 13538.91]& [13537.05 , 13539.50]& [13536.05 , 13540.00]\\ lin.smoothed rhk& -1.074719& -1.392857& -1.409786& [-1.884 , -0.861]& [-2.413 , -0.353]& [-2.88 , 0.13]\\ \hline  \multicolumn{7}{c}{Planet1}\\ \hline$P$ (d)& 3.4303077& 3.4307496& 3.4307133& [3.4296 , 3.4315]& [3.4288 , 3.4327]& [3.4280 , 3.4339]\\ $K$ (m/s) & 1.85672& 2.06798& 2.06598& [1.85 , 2.28]& [1.64 , 2.53]& [1.50 , 2.72]\\ $\lambda_0$ (rad) & 3.24354& 3.45104& 3.42827& [2.88 , 3.87]& [2.40 , 4.49]& [1.99 , 5.11]\\ $\sqrt{e} \cos \omega$ & -0.16399& -0.00403& -0.00607& [-0.08 , 0.08]& [-0.14 , 0.17]& [-0.23 , 0.23]\\ $\sqrt{e} \sin \omega$ & -0.01251& 0.00190& 0.00104& [-0.07 , 0.09]& [-0.17 , 0.16]& [-0.22 , 0.27]\\ \hline  \multicolumn{7}{c}{Planet2}\\ \hline$P$ (d)& 5.1998109& 5.1992000& 5.1992032& [5.1974 , 5.2013]& [5.1950 , 5.2031]& [5.192 , 5.205]\\ $K$ (m/s) & 2.50034& 2.29807& 2.29293& [2.08 , 2.51]& [1.87 , 2.75]& [1.69 , 3.03]\\ $\lambda_0$ (rad) & 5.37377& 5.14144& 5.16235& [4.77 , 5.58]& [4.27 , 5.97]& [0.03 , 6.19]\\ $\sqrt{e} \cos \omega$ & 0.21109& -0.01898& -0.01967& [-0.08 , 0.04]& [-0.16 , 0.09]& [-0.22 , 0.19]\\ $\sqrt{e} \sin \omega$ & -0.02838& 0.01729& 0.01815& [-0.05 , 0.09]& [-0.13 , 0.17]& [-0.23 , 0.23]\\ \hline  \multicolumn{7}{c}{Planet3}\\ \hline$P$ (d)& 7.943203& 7.944831& 7.944719& [7.938 , 7.951]& [7.933 , 7.957]& [7.923 , 7.965]\\ $K$ (m/s) & 2.12079& 1.86638& 1.87138& [1.57 , 2.14]& [1.27 , 2.48]& [1.05 , 2.86]\\ $\lambda_0$ (rad) & 2.39500& 2.56982& 2.56625& [2.07 , 3.26]& [1.37 , 3.72]& [0.72 , 4.67]\\ $\sqrt{e} \cos \omega$ & -0.03171& -0.01302& -0.01148& [-0.07 , 0.04]& [-0.12 , 0.11]& [-0.22 , 0.15]\\ $\sqrt{e} \sin \omega$ & 0.08663& 0.00728& 0.01032& [-0.05 , 0.08]& [-0.14 , 0.14]& [-0.20 , 0.23]\\ \hline  \multicolumn{7}{c}{Planet4}\\ \hline$P$ (d)& 12.0307146& 12.0229496& 12.0246362& [12.002 , 12.048]& [11.970 , 12.069]& [11.94 , 12.09]\\ $K$ (m/s) & 2.30081& 2.37814& 2.38840& [2.04 , 2.71]& [1.68 , 3.08]& [1.25 , 3.40]\\ $\lambda_0$ (rad) & 6.11898& 4.05252& 5.10616& [4.16 , 6.28]& [0.12 , 6.28]& [0.00 , 6.28]\\ $\sqrt{e} \cos \omega$ & -0.07610& -0.02329& -0.02342& [-0.08 , 0.04]& [-0.15 , 0.11]& [-0.21 , 0.18]\\ $\sqrt{e} \sin \omega$ & 0.06347& 0.01315& 0.00872& [-0.07 , 0.08]& [-0.13 , 0.18]& [-0.20 , 0.24]\\ \hline 

 \multicolumn{7}{c}{Planet5}\\ \hline$P$ (d)& 17.2729662& 17.2953069& 17.2960144& [17.252 , 17.344]& [17.19 , 17.39]& [17.16 , 17.44]\\ $K$ (m/s) & 2.13460& 2.50230& 2.49632& [2.12 , 2.99]& [1.70 , 3.40]& [0.89 , 3.72]\\ $\lambda_0$ (rad) & 6.13717& 2.66307& 1.40828& [0.00 , 5.09]& [0.09 , 6.25]& [0.00 , 6.27]\\ $\sqrt{e} \cos \omega$ & 0.01815& -0.01578& -0.01688& [-0.10 , 0.05]& [-0.17 , 0.14]& [-0.25 , 0.22]\\ $\sqrt{e} \sin \omega$ & 0.05519& -6.13611& 0.00130& [-0.06 , 0.08]& [-0.13 , 0.14]& [-0.21 , 0.20]\\ \hline  

\multicolumn{7}{c}{Planet6}\\ \hline$P$ (d)& 365.5631857& 365.0360385& 365.0280150& [364.24 , 365.57]& [363.82 , 366.40]& [363.29 , 366.86]\\ $K$ (m/s) & 0.08329& 0.91412& 0.75597& [0.01 , 1.13]& [0.00 , 2.35]& [0.00 , 3.85]\\ $\lambda_0$ (rad) & 5.02441& 3.13689& 2.94889& [1.46 , 5.49]& [0.24 , 6.14]& [0.01 , 6.27]\\ $\sqrt{e} \cos \omega$ & -0.17301& -0.00394& -0.00724& [-0.06 , 0.06]& [-0.13 , 0.14]& [-0.20 , 0.21]\\ $\sqrt{e} \sin \omega$ & 0.01805& -0.01798& -0.01930& [-0.10 , 0.04]& [-0.16 , 0.14]& [-0.22 , 0.27]\\ \hline  \multicolumn{7}{c}{Planet7}\\ \hline$P$ (d)& 2.17830038& 2.17824579& 2.17826547& [2.17776 , 2.17871]& [2.1772 , 2.1792]& [2.1767 , 2.1796]\\ $K$ (m/s) & 0.77507& 0.74807& 0.76458& [0.55 , 0.97]& [0.24 , 1.19]& [0.00 , 1.39]\\ $\lambda_0$ (rad) & 1.50015& 1.84387& 1.77027& [1.03 , 2.42]& [0.10 , 3.33]& [0.00 , 6.00]\\ $\sqrt{e} \cos \omega$ & -0.10655& 0.01961& 0.01692& [-0.07 , 0.09]& [-0.15 , 0.18]& [-0.22 , 0.29]\\ $\sqrt{e} \sin \omega$ & -0.05719& 0.00906& 0.01023& [-0.06 , 0.07]& [-0.13 , 0.14]& [-0.21 , 0.20]\\ \hline  \multicolumn{7}{c}{Planet8}\\ \hline$\sigma_W$ (d)& 0.11910& 0.71020& 0.71716& [0.44 , 0.97]& [0.11 , 1.23]& [0.01 , 1.52]\\ $\sigma_R$ (d)& 9.28659& 3.46716& 3.47634& [3.17 , 3.76]& [2.91 , 4.11]& [2.56 , 4.28]\\ $\tau$ (d)& 6.18576& 7.70776& 7.28137& [4.96 , 8.86]& [4.139 , 12.65]& [3.51 , 18.1]\\ 
$m\sin i$ ($M_\oplus$)& 4.60& 5.11& 5.06& [4.44 , 5.69]& [3.97 , 6.42]& [3.56 , 7.21]\\ 
$m\sin i$ ($M_\oplus$)& 7.12& 6.53& 6.47& [5.75 , 7.23]& [5.10 , 8.14]& [4.29 , 8.68]\\ 
$m\sin i$ ($M_\oplus$)& 6.96& 6.11& 6.12& [5.11 , 7.16]& [4.06 , 8.34]& [3.24 , 9.81]\\ 
$m\sin i$ ($M_\oplus$)& 8.675& 8.939& 8.959& [7.559 , 10.32]& [6.175 , 11.91]& [4.937 , 13.54]\\ 
$m\sin i$ ($M_\oplus$)& 9.079& 10.61& 10.55& [8.668 , 12.63]& [7.116 , 14.82]& [3.84 , 15.9]\\ 
$m\sin i$ ($M_\oplus$)& 0.97& 10.7& 8.88& [0.24 , 13.4]& [0.01 , 27.8]& [0.01 , 45.0]\\ 
$m\sin i$ ($M_\oplus$)& 1.65& 1.58& 1.61& [1.13 , 2.05]& [0.46 , 2.53]& [0.00 , 2.89]\\ 

==> parameters_evolution_pfixed.tex <==
Parameter & ML fit & posterior mean & posterior median & 68.27\% confidence interval & 95.45\% confidence interval & 99.73\% confidence interval\\ \hline \hline  lin.offset& 13536.434739433& 13536.850673545& 13536.821345451& [13536.23 , 13537.37]& [13535.72 , 13538.15]& [13534.90 , 13539.07]\\ lin.smoothed rhk& -3.334304& -3.450329& -3.461636& [-3.984 , -2.885]& [-4.611 , -2.346]& [-5.223 , -1.810]\\ \hline  \multicolumn{7}{c}{Planet1}\\ \hline$P$ (d)& 3.4319607& 3.4319958& 3.4319766& [3.4309 , 3.4329]& [3.4301 , 3.4339]& [3.4292 , 3.4348]\\ $K$ (m/s) & 2.61357& 2.54714& 2.54274& [2.18 , 2.81]& [1.93 , 3.17]& [1.59 , 3.57]\\ $\lambda_0$ (rad) & 4.25605& 4.25004& 4.25123& [4.12 , 4.37]& [3.97 , 4.49]& [3.85 , 4.66]\\ $\sqrt{e} \cos \omega$ & -0.00563& 0.01746& 0.01612& [-0.07 , 0.09]& [-0.15 , 0.20]& [-0.27 , 0.28]\\ $\sqrt{e} \sin \omega$ & -0.08176& -0.00281& -0.00241& [-0.09 , 0.08]& [-0.17 , 0.18]& [-0.29 , 0.27]\\ \hline  \multicolumn{7}{c}{Planet2}\\ \hline$P$ (d)& 5.209166& 5.205985& 5.206134& [5.200 , 5.212]& [5.193 , 5.218]& [5.181 , 5.224]\\ $K$ (m/s) & 1.17545& 1.18443& 1.19650& [0.84 , 1.56]& [0.44 , 1.91]& [0.02 , 2.15]\\ $\lambda_0$ (rad) & 5.23518& 4.95749& 4.98189& [4.63 , 5.33]& [4.21 , 5.77]& [0.56 , 6.26]\\ $\sqrt{e} \cos \omega$ & -0.02341& 0.00342& 0.00420& [-0.08 , 0.08]& [-0.16 , 0.19]& [-0.27 , 0.27]\\ $\sqrt{e} \sin \omega$ & 0.01262& -0.00901& -0.01170& [-0.09 , 0.07]& [-0.17 , 0.18]& [-0.26 , 0.29]\\ \hline  \multicolumn{7}{c}{Planet3}\\ \hline$P$ (d)& 7.952462& 7.944880& 7.944952& [7.936 , 7.953]& [7.925 , 7.962]& [7.913 , 7.980]\\ $K$ (m/s) & 1.64134& 1.53601& 1.55113& [1.10 , 1.95]& [0.63 , 2.39]& [0.01 , 2.69]\\ $\lambda_0$ (rad) & 3.71881& 3.49416& 3.50804& [3.22 , 3.78]& [2.83 , 4.05]& [2.23 , 4.52]\\ $\sqrt{e} \cos \omega$ & -0.07124& -0.00365& -0.00120& [-0.08 , 0.09]& [-0.17 , 0.18]& [-0.27 , 0.25]\\ $\sqrt{e} \sin \omega$ & -0.02711& -0.00419& -0.00128& [-0.08 , 0.08]& [-0.18 , 0.17]& [-0.27 , 0.25]\\ \hline  \multicolumn{7}{c}{Planet4}\\ \hline$P$ (d)& 12.0381121& 12.0301462& 12.0291288& [12.001 , 12.057]& [11.97 , 12.09]& [11.92 , 12.13]\\ $K$ (m/s) & 1.52184& 1.03811& 1.01033& [0.39 , 1.58]& [0.00 , 2.00]& [0.00 , 2.61]\\ $\lambda_0$ (rad) & 2.29184& 4.68232& 5.06416& [4.53 , 5.93]& [0.44 , 6.28]& [0.00 , 6.27]\\ $\sqrt{e} \cos \omega$ & -0.02825& -0.01621& -0.01514& [-0.10 , 0.06]& [-0.19 , 0.14]& [-0.29 , 0.26]\\ $\sqrt{e} \sin \omega$ & -0.13556& -0.00144& 0.00083& [-0.08 , 0.09]& [-0.19 , 0.18]& [-0.30 , 0.27]\\ \hline  \multicolumn{7}{c}{Planet5}\\ \hline$P$ (d)& 17.649819& 17.548409& 17.557139& [17.51 , 17.62]& [17.41 , 17.66]& [17.31 , 17.70]\\ $K$ (m/s) & 2.19049& 1.91128& 1.93167& [1.43 , 2.49]& [0.64 , 3.02]& [0.00 , 3.50]\\ $\lambda_0$ (rad) & 4.34062& 3.80909& 3.86115& [3.52 , 4.24]& [2.86 , 4.58]& [1.07 , 5.01]\\ $\sqrt{e} \cos \omega$ & 0.09226& -0.00126& -0.00065& [-0.08 , 0.08]& [-0.17 , 0.17]& [-0.29 , 0.26]\\ $\sqrt{e} \sin \omega$ & -0.05751& 0.00624& 0.00733& [-0.08 , 0.10]& [-0.17 , 0.20]& [-0.26 , 0.28]\\ \hline  \multicolumn{7}{c}{Planet6}\\ \hline$P$ (d)& 363.8396112& 365.0428204& 365.0555666& [364.21 , 365.93]& [363.27 , 366.79]& [362.59 , 367.76]\\ $K$ (m/s) & 1.60189& 1.22618& 1.09765& [0.01 , 1.55]& [0.00 , 2.84]& [0.00 , 4.12]\\ $\lambda_0$ (rad) & 2.68801& 2.95045& 2.90054& [1.97 , 3.83]& [0.19 , 5.20]& [0.01 , 6.17]\\ $\sqrt{e} \cos \omega$ & 0.15089& 0.00425& 0.00331& [-0.09 , 0.08]& [-0.18 , 0.18]& [-0.26 , 0.27]\\ $\sqrt{e} \sin \omega$ & 0.12374& -0.00067& -0.00087& [-0.10 , 0.08]& [-0.18 , 0.19]& [-0.28 , 0.27]\\ \hline  \multicolumn{7}{c}{Planet7}\\ \hline$P$ (d)& 2.1788531& 2.1782462& 2.1782417& [2.1776 , 2.1788]& [2.1771 , 2.1794]& [2.1765 , 2.1798]\\ $K$ (m/s) & 0.78185& 1.03309& 1.03585& [0.75 , 1.30]& [0.47 , 1.61]& [0.07 , 1.87]\\ $\lambda_0$ (rad) & 0.73799& 0.87504& 0.60348& [0.20 , 0.86]& [1.36 , 5.90]& [0.00 , 6.27]\\ $\sqrt{e} \cos \omega$ & -0.00781& 0.01189& 0.01216& [-0.06 , 0.10]& [-0.16 , 0.19]& [-0.26 , 0.28]\\ $\sqrt{e} \sin \omega$ & 0.04206& -0.00142& -0.00144& [-0.09 , 0.09]& [-0.19 , 0.18]& [-0.28 , 0.27]\\ \hline  \multicolumn{7}{c}{Planet8}\\ \hline$\sigma_W$ (d)& 0.15445& 0.91944& 0.92170& [0.55 , 1.34]& [0.16 , 1.64]& [0.03 , 2.03]\\ $\sigma_R$ (d)& 9.62517& 3.34839& 3.32940& [2.93 , 3.68]& [2.60 , 4.18]& [2.29 , 4.68]\\ $\tau$ (d)& 3.13502& 4.24749& 3.81007& [2.46 , 4.89]& [1.76 , 8.05]& [1.53 , 13.4]\\ 
$m\sin i$ ($M_\oplus$)& 6.48& 6.30& 6.28& [5.42 , 7.15]& [4.48 , 8.02]& [3.79 , 8.96]\\ 
$m\sin i$ ($M_\oplus$)& 3.35& 3.37& 3.37& [2.28 , 4.37]& [1.12 , 5.45]& [0.03 , 6.23]\\ 
$m\sin i$ ($M_\oplus$)& 5.39& 5.03& 5.06& [3.61 , 6.46]& [2.27 , 8.19]& [0.42 , 9.17]\\ 
$m\sin i$ ($M_\oplus$)& 5.73& 3.90& 3.80& [1.52 , 6.01]& [0.00 , 7.65]& [0.00 , 10.3]\\ 
$m\sin i$ ($M_\oplus$)& 9.384& 8.153& 8.205& [6.085 , 10.76]& [2.86 , 13.2]& [0.03 , 15.4]\\ 
$m\sin i$ ($M_\oplus$)& 18.8& 14.4& 12.8& [0.04 , 18.0]& [0.04 , 33.8]& [0.02 , 48.7]\\ 
$m\sin i$ ($M_\oplus$)& 1.66& 2.19& 2.20& [1.59 , 2.78]& [0.91 , 3.39]& [0.17 , 4.08]\\ 














Parameter & ML fit & posterior mean & posterior median & 68.27\% confidence interval & 95.45\% confidence interval & 99.73\% confidence interval\\ \hline \hline  lin.offset& 13538.165098098& 13538.595051722& 13538.613524010& [13537.68 , 13539.65]& [13536.44 , 13540.46]& [13535.50 , 13541.89]\\ lin.smoothed rhk& 1.08352& 0.86581& 0.86762& [0.16 , 1.53]& [-0.52 , 2.37]& [-1.78 , 3.30]\\ \hline  \multicolumn{7}{c}{Planet1}\\ \hline$P$ (d)& 3.4353604& 3.4352882& 3.4353243& [3.4339 , 3.4366]& [3.4326 , 3.4381]& [3.4307 , 3.4393]\\ $K$ (m/s) & 1.88719& 2.07725& 2.08164& [1.80 , 2.35]& [1.48 , 2.65]& [1.10 , 2.97]\\ $\lambda_0$ (rad) & 0.84061& 2.41480& 1.62247& [0.00 , 2.63]& [0.14 , 6.27]& [0.00 , 6.27]\\ $\sqrt{e} \cos \omega$ & 0.01995& 0.01217& 0.01175& [-0.08 , 0.11]& [-0.18 , 0.20]& [-0.28 , 0.29]\\ $\sqrt{e} \sin \omega$ & 0.08887& 0.00975& 0.01061& [-0.08 , 0.11]& [-0.18 , 0.22]& [-0.30 , 0.31]\\ \hline  \multicolumn{7}{c}{Planet2}\\ \hline$P$ (d)& 5.2037914& 5.2037031& 5.2037304& [5.2005 , 5.2073]& [5.196 , 5.210]& [5.192 , 5.214]\\ $K$ (m/s) & 2.36889& 2.16315& 2.17284& [1.84 , 2.55]& [1.38 , 2.89]& [1.03 , 3.28]\\ $\lambda_0$ (rad) & 0.66572& 2.55540& 1.72033& [0.00 , 3.37]& [0.04 , 6.15]& [0.00 , 6.26]\\ $\sqrt{e} \cos \omega$ & 0.15716& 0.02006& 0.01650& [-0.09 , 0.11]& [-0.19 , 0.23]& [-0.27 , 0.37]\\ $\sqrt{e} \sin \omega$ & -0.15045& -0.02038& -0.01778& [-0.11 , 0.07]& [-0.21 , 0.17]& [-0.33 , 0.26]\\ \hline  \multicolumn{7}{c}{Planet3}\\ \hline$P$ (d)& 7.958730& 7.963588& 7.963800& [7.956 , 7.970]& [7.947 , 7.977]& [7.937 , 7.990]\\ $K$ (m/s) & 2.54148& 2.45758& 2.45684& [2.08 , 2.92]& [1.56 , 3.27]& [1.03 , 3.74]\\ $\lambda_0$ (rad) & 4.75029& 3.97261& 4.75111& [3.70 , 6.28]& [0.16 , 6.24]& [0.01 , 6.28]\\ $\sqrt{e} \cos \omega$ & 0.06434& -0.01473& -0.01507& [-0.11 , 0.07]& [-0.20 , 0.18]& [-0.30 , 0.25]\\ $\sqrt{e} \sin \omega$ & 0.00165& 0.01883& 0.01970& [-0.08 , 0.11]& [-0.17 , 0.21]& [-0.27 , 0.29]\\ \hline  \multicolumn{7}{c}{Planet4}\\ \hline$P$ (d)& 12.0315752& 12.0193243& 12.0188270& [11.989 , 12.042]& [11.96 , 12.07]& [11.92 , 12.12]\\ $K$ (m/s) & 1.37611& 1.33991& 1.33639& [0.84 , 1.86]& [0.26 , 2.34]& [0.00 , 2.89]\\ $\lambda_0$ (rad) & 5.58856& 3.48048& 3.74122& [2.70 , 6.20]& [0.11 , 6.04]& [0.01 , 6.26]\\ $\sqrt{e} \cos \omega$ & -0.06128& 0.00074& 0.00299& [-0.09 , 0.09]& [-0.20 , 0.18]& [-0.27 , 0.25]\\ $\sqrt{e} \sin \omega$ & 0.01748& -0.00674& -0.00684& [-0.10 , 0.09]& [-0.20 , 0.19]& [-0.34 , 0.25]\\ \hline  \multicolumn{7}{c}{Planet5}\\ \hline$P$ (d)& 17.274824& 17.324761& 17.321861& [17.26 , 17.37]& [17.20 , 17.43]& [17.16 , 17.53]\\ $K$ (m/s) & 1.99048& 1.81737& 1.82069& [1.17 , 2.37]& [0.40 , 2.93]& [0.01 , 3.68]\\ $\lambda_0$ (rad) & 4.09034& 3.40018& 3.73650& [2.17 , 6.28]& [0.25 , 6.27]& [0.00 , 6.27]\\ $\sqrt{e} \cos \omega$ & 0.05827& 0.00304& 0.00202& [-0.09 , 0.10]& [-0.18 , 0.20]& [-0.30 , 0.27]\\ $\sqrt{e} \sin \omega$ & 0.06123& -0.00597& -0.00767& [-0.11 , 0.07]& [-0.21 , 0.19]& [-0.29 , 0.29]\\ \hline  \multicolumn{7}{c}{Planet6}\\ \hline$P$ (d)& 363.6774902& 364.9919011& 364.9763067& [363.97 , 365.66]& [363.38 , 366.90]& [362.34 , 367.81]\\ $K$ (m/s) & 3.07980& 2.45518& 2.41876& [1.23 , 3.75]& [0.11 , 4.78]& [0.00 , 6.43]\\ $\lambda_0$ (rad) & 2.46357& 2.89529& 2.80343& [2.19 , 3.27]& [1.61 , 4.57]& [0.49 , 6.18]\\ $\sqrt{e} \cos \omega$ & -0.11529& -0.00908& -0.00823& [-0.09 , 0.09]& [-0.21 , 0.19]& [-0.33 , 0.27]\\ $\sqrt{e} \sin \omega$ & 0.00428& -0.00543& -0.00554& [-0.11 , 0.09]& [-0.23 , 0.18]& [-0.30 , 0.32]\\ \hline  \multicolumn{7}{c}{Planet7}\\ \hline$P$ (d)& 2.1785563& 2.1783578& 2.1783635& [2.1778 , 2.1788]& [2.1773 , 2.1794]& [2.1767 , 2.1799]\\ $K$ (m/s) & 1.06036& 1.11386& 1.13048& [0.82 , 1.44]& [0.40 , 1.74]& [0.07 , 2.06]\\ $\lambda_0$ (rad) & 1.87525& 2.05766& 1.73856& [0.20 , 2.42]& [0.02 , 5.85]& [0.02 , 6.28]\\ $\sqrt{e} \cos \omega$ & 0.03574& 0.01377& 0.01401& [-0.09 , 0.10]& [-0.18 , 0.20]& [-0.29 , 0.30]\\ $\sqrt{e} \sin \omega$ & -0.04711& 0.00545& 0.00455& [-0.08 , 0.10]& [-0.18 , 0.20]& [-0.32 , 0.31]\\ \hline  \multicolumn{7}{c}{Planet8}\\ \hline$\sigma_W$ (d)& 1.41796& 1.01592& 1.00602& [0.64 , 1.40]& [0.18 , 1.77]& [0.04 , 2.31]\\ $\sigma_R$ (d)& 6.94797& 3.22725& 3.19192& [2.68 , 3.60]& [2.28 , 4.23]& [1.91 , 5.18]\\ $\tau$ (d)& 7.87946& 8.18853& 6.83190& [3.37 , 9.03]& [2.17 , 18.6]& [2.17 , 27.7]\\ 
$m\sin i$ ($M_\oplus$)& 4.68& 5.15& 5.13& [4.40 , 5.92]& [3.51 , 6.65]& [2.83 , 7.83]\\ 
$m\sin i$ ($M_\oplus$)& 6.74& 6.15& 6.14& [5.16 , 7.34]& [3.76 , 8.29]& [2.67 , 9.78]\\ 
$m\sin i$ ($M_\oplus$)& 8.34& 8.06& 8.07& [6.63 , 9.55]& [4.959 , 10.95]& [3.294 , 12.84]\\ 
$m\sin i$ ($M_\oplus$)& 5.18& 5.04& 5.03& [3.08 , 6.95]& [0.94 , 8.79]& [0.02 , 10.8]\\ 
$m\sin i$ ($M_\oplus$)& 8.467& 7.724& 7.705& [5.164 , 10.37]& [2.14 , 12.9]& [0.06 , 15.6]\\ 
$m\sin i$ ($M_\oplus$)& 36.1& 28.8& 28.3& [14.1 , 44.2]& [0.88 , 55.8]& [0.03 , 76.1]\\ 
$m\sin i$ ($M_\oplus$)& 2.26& 2.37& 2.37& [1.70 , 3.06]& [0.85 , 3.75]& [0.07 , 4.37]\\ 
